On the Benefits And Problems Related to Using Definition of Done -- A Survey Study

Context: Definition of Done (DoD) is one of the fundamental concepts of Scrum. It expresses a shared view of a Scrum Team on what makes an increment of their product complete. DoDs are often defined as checklists with items being requirements towards software (e.g., quality requirements) or towards activities performed to make the increment shippable (e.g., code reviews, testing). Unfortunately, the knowledge about the usefulness of DoD is still very limited. Objective: The goal is to study what benefits using the DoD practice can bring to an agile project, what problems it may trigger, and how it is created and maintained. Method: In the survey among members of agile software development projects, 137 practitioners from all over the globe shared their experience with us. Results: 93% of the respondents perceive DoD as at least valuable for their ventures. It helps them to make work items complete, assure product quality, and ensure the needed activities are executed. However, they indicated that every second project struggles with infeasible, incorrect, unavailable, or creeping DoD. Conclusions: It follows from the study that DoD is important but not easy to use and more empirical studies are needed to identify best practices in this area.

==> discussion-old.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{RQ1. What are the benefits of using DoD?}

The results of the survey show that using DoD is perceived as a useful practice. The respondents of the survey nearly unanimously (ca. 93\% of respondents) agreed that using DoD brings value to agile projects. From the nineteen benefits of using DoD that we asked the respondents about, only one was present in less than half of the projects. 

The benefits that should materialize in nearly every project using DoD (appeared in ca. 90\% or more projects in our study) are directly following from the purpose of DoD itself, i.e., ensuring the completeness of work items and ensuring the expected level of product quality (e.g., by ensuring that all activities other than coding are executed and all quality gates are passed). \abc{We also observed that these benefits are highly correlated. Therefore, it is rather unlikely to expect or see that either of them materialize without the rest of them.}

Another group of common benefits regards helping to increase predictability and transparency in a project (e.g., supporting effort estimation, allowing for the common understanding of what ``complete'' means, and ensuring that organization standards are used). Also, in ca. 60\% of cases having a DoD defined allowed to improve teams' productivity (e.g., by reducing the time needed to rework). Moreover, the use of DoD increases the overall quality of software products as it reduces technical debt and the number of defects in the code. \abc{The correlation analysis revealed strong correlation between benefits regarding code transparency and code quality.} Finally, DoD can translate into increased customer satisfaction \abc{(also by reducing the number of defects being released)}. 



On contrary, the projects that did not define DoDs struggle with problems that are the inverse of the benefits discussed above (e.g., technical problems related to defects, low quality, or technical debt). Lack of agreed understanding of what ``Done'' means might  negatively affect teamwork and lead to misunderstandings and problems with assigning responsibilities. Finally, at the project level, the lack of DoD can lead to missing deadlines, poor quality, chaos, and ultimately to stakeholders' dissatisfaction.   


\subsection{RQ2. What are the problems encountered while using DoD and how they are mitigated?}

%Using DoD in a project, like any other practice, brings additional costs and triggers some difficulties that the project team need to solve in order to benefit from using it. In our study, we asked participants to evaluate the frequency and significance of nineteen problems related to using the DoD practice. 

Using DoD in a project, like any other practice, brings additional costs and triggers some difficulties that the project team needs to overcome to benefit from using it.
The results of our study show that the problems related to DoD are common and appeared in at least 40\% of the projects. We could classify most of them as moderately harmful since only in 1/3 to 1/2 of the projects the respondents assessed their negative impact on the project as significant. However, this is still surprisingly high when we consider how basic the practice of defining a DoD may seem.  The most important problems with using DoDs are very similar to those characteristic for specifying product requirements, i.e., lack of precision, ambiguity, incompleteness, infeasibility, or difficulty in getting acceptance by stakeholders.

Although agile teams often rely on oral communication, the results of the study show that it is worth considering investing time and resources in documenting a DoD and making it available to all team members. The lack of thereof was indicated by the respondents as the most significant problem related to DoD (fortunately, also one of the less frequently appearing). On contrary, the respondents indicated the problems related to the costs of creating and using the DoD to verify work items were as one of the most frequently appearing. However, they were most often evaluated as non-significantly harmful. 
 
%Finally, the changes in DoD were also considered as problems by the respondents, however, we do not know whether it was the deterioration of the existing items or the necessity of adding new ones causing the problems. 

Regarding the means of overcoming the aforementioned problems, it seems that there are no systematic and dedicated methods. According to the respondents, the only way to tackle most of the problems regarding DoD is to talk them over by the team (sometimes with the help of an agile coach or Scrum Master).
 
\subsection{RQ3. How is a DoD established and maintained?}

The results of our survey did not reveal the presence of a single, agreed process of creating DoDs in agile projects. However, there are some common steps and tools that are widely used by agile teams that we could combine into a broader, generic DoD life-cycle process. 

In our study, we made similar observations to Silva et al. \cite{Silva2018} that DoDs are usually created employing teamwork activities (e.g., brainstorming techniques or discussion).  However, we also observed that some organizations support this step by re-using knowledge from previous projects, either by maintaining and using DoD templates or organization standards. Also, some of the respondents emphasized the need of analyzing and adjusting the proposed DoD before it is put into use to clarify ambiguities, assess the feasibility of DoD items, or prioritize the DoD items. 

As soon as the DoD reaches its agreed, initial version, it is made accessible to the project team. We identified two main channels for sharing DoDs. The most popular way is to use electronic tools for this purpose, e.g., web pages, wiki, or task-management systems (the same was reported by Silva et al. \cite{Silva2018}), while the second most popular way is to use a physical copy of DoD and hang it on the wall in the team's office. Finally, it seems that the most preferred way of documenting DoDs is to express them in the form of checklists or ``tickets'' in task management systems. Interestingly, DoD might also become a part of a code review procedure as a part of the pull-request template.


DoDs are project-long living artifacts. They are often created before or at the initial stages of projects and regularly evaluated and updated, either on some agreed intervals or on-demand. Nevertheless, in the case of ca. 11\% of the studied projects, their DoDs were never updated, which means that they were valid and complete from the beginning to the end, or the practice was abandoned at some point. 

Finally, DoDs are mainly created by Developers, Product Owners, and Scrum Masters. However, it is not an uncommon situation that a DoD is created without the involvement of developers (22\%), which we find as a surprising and counterintuitive observation. 


\subsection{Implications to research}

Our study confirms that using DoDs is useful, what has been already claimed by several researchers and practitioners based on their experience, e.g., \cite{Saddington2012}, \cite{jakobsen2008mature}, \cite{cohn2010succeeding}. 

We identified and evaluated the importance of several benefits that DoDs might bring. However, our findings are a trigger for opening a new discussion about when such benefits are present and how to create an effective DoD to help materialize these benefits.

Our study extends the body of knowledge related to the problems encountered while using DoDs by providing an initial evaluation of their frequency and significance. Since several problems might appear frequently and have a negative impact on agile projects, a further and more in-depth analysis would be valuable. We identify an opportunity for more fine-grained research on why the problems appear, what we can do to prevent them, and how to solve them.
 
%As we found in our literature review, there are a few studies that report problems concerning DoDs, e.g., \cite{OConnor2010}, \cite{Igaki2014}.

Also, the results of the survey complement the previous studies on investigating how the practice of DoD is applied, e.g., \cite{Silva2017}, \cite{Silva2018}. The respondents reported that there are multiple ways of creating and maintaining DoDs. Therefore, as future research, it would be worth investigating the advantages and disadvantages of different approaches.

% e.g., various roles take care of DoD, counter-intuitively sometimes Developers do not establish DoD, sometimes DoD is established at the beginning of the project and another time in multiple rounds. Since there is no single way how to use DoD, it is worth investigating what the advantages and disadvantages of each approach are.

Moreover, new research directions are opened by two groups of problems---the problems related to the specification of DoDs and the cost of creating and maintaining DoD. It would be worth considering the possibility of supporting or even automating to some degree the process of creating DoDs. 

Finally, from the empirical software engineering perspective, we would like to draw the attention of other researchers to the usability of the questionnaire used in their survey, especially the presentation of the questions. It might have a significant impact on the response rate. It follows from the analysis of the drop-outs in our study that a significant number of our respondents left when they were presented a list of benefits or a list of problems to assess (i.e., a list of several items to assess on a scale with more than 5 values). It seems that it might be caused by the presentation method of the list-type of questions, e.g., the impression that answering the question would be overwhelming or time-consuming.  

%Since using DoD is an agile practice and DoD constitute of items which are requirements, it seems valuable to start the investigation by validating the already existing RE practices used in agile projects.

%co tu napisac?
%- jest wazna tak jak sugeruja inni [] i rozszerzamy o systamtycza identyfikacje benefitow
%- jak wynika z literatury istnieje malo zidentyfikowanych problemow, my rozszerzamy 
%i pokazujemy ze konkretne problemy wystepuja dosc czesto i moga miec spore znaczenie, stad glebsza analiza %bylaby bardzo ciekawa 
%- pokazujemy jak ludzie tworza i utrzymuja DoD. Rozszerzamy to co napisala Silva i wydaje sie ze nie ma %jednego sprawdzonego sposobu tak, ciekawe by bylo zbadanie ktora technika jest najbardziej efektywana, %dlaczego i w jakim kontekscie
%Our results suggest that 
%However, existing research 

\subsection{Implications for practitioners}
Our findings show that the DoD practice is perceived as useful by nearly all practitioners who used it. The primary benefits are about helping to make work items complete to ensure product quality and that the activities other than coding are executed, and all quality gates are passed to keep the product releasable. 

However, when deciding to use DoD or when thinking about improving that practice, one needs to understand that there might appear some problems along the way. The list of problems and their evaluation from the frequency and significance perspectives might help practitioners to assess the risks related to adopting the DoD practice and prepare in advance.


%The problems might be related to how a team create and use their DoD, e.g., high effort of creating a DoD or to verify if it is satisfied, and differences in understanding its items. Moreover, there might be some problems with formulating DoD like missing, unclear, or impossible to verify DoD. Unfortunately, those problems appear quite frequently and might significantly negatively impact a project. However, the proven techniques to solve the problems include mainly team cooperation (e.g., workshops, brainstorming sessions) which not only would improve the DoD practice, but might positively impact how team work together.  Sometimes, however, help from more knowledgeable persons like coach can be the solution.

It is also important to be aware of the fact that when a team dismisses to use DoD in their project, several important risks might materialize, such as, not meeting the deadline, lack of shared understanding of what ``done'' means, defects, low quality, and technical debt.

Finally, the results of our study show how practitioners establish and maintain DoD  which can be used for educational proposes. It might be especially useful for novice Scrum adepts who look for guidelines on preparing a DoD or for those who look for some ideas on how to improve their process. Moreover, together with the information about the benefits, it might provide a strong argument in favor of using DoD for those who are reluctant (e.g., for Scrum Masters or agile coaches who would like to convince those undecided).

%Therefore, these observations seem to confirm the observations made while analyzing the \emph{Significance} measure that the problems related to how DoD is formulated are of big importance.


==> mrcv.tex <==
\subsection{Relationships with context}

\begin{figure*}
\centerline{\includegraphics[width=\textwidth]{mrcvProblems.pdf}}
\caption{How DoDs are created and maintained?}
\label{fig:how}
\end{figure*}

When Developers take part in creating DoD several problems related to how DoD is used (P2, P11, P12) and with infeasibility of DoD items (P19) are claimed to do not appear more frequently. When some problems like P4, P8, P15, P19 do appear in those projects less frequently they are perceived as significant. What is interesting is that when Developers are involved in establishing DoD more frequently the problem of changing DoD (P13) is perceived as significant. 
The problem P4 with defining universal DoD is perceived as significant more frequently in large organizations.
When DoD was not documented the problems with imprecise (P5), missing (6), impossible to be verified (P8) DoD items were more frequently identified as significant comparing to when it was documented and persisted in other forms like in team management system etc. 
The problem concerning verification of DoD items (P8) seems to appear more frequently then it is not documented, but less frequently when it is on an office wall. Moreover it seems to have more frequently a significant impact for bitter teams.
Significance of some problems seem to depend on the size of organization. Problems concerning the effort of verification of DoD items (P3) and difficulties to understand them were reported less frequently significant and more frequently not significant in medium size organizations. While defining universal DoD (P4) and DoD items that were impossible to be verified (P8) appeared more frequently significant in large scale organizations.
Interestingly, when there were over 3 nationalities the fact that DoD was not documented (P17) was identified as problem did not appeared more frequently than when there were fewer nationalities in projects. But the high number of nationalities was identified more frequently. However, the respondents did not reach consensus (there was 50\%/50\%) if it has or has not a significant negative impact on the project.
Experience of respondents  both general and in agile projects seem to influence how problems are perceived. Those with high experience (over 5 years) identified several problems (P4, P8, P9, P14, P15) less frequently and in majority of cases they more frequently regarded them as not significant.

